GarmentImage: Raster Encoding of Garment Sewing Patterns with Diverse Topologies

Garment sewing patterns are the design language behind clothing, yet their current vector-based digital representations weren't built with machine learning in mind. Vector-based representation encodes a sewing pattern as a discrete set of panels, each defined as a sequence of lines and curves, stitching information between panels and the placement of each panel around a body. However, this representation causes two major challenges for neural networks: discontinuity in latent space between patterns with different topologies and limited generalization to garments with unseen topologies in the training data. In this work, we introduce GarmentImage, a unified raster-based sewing pattern representation. GarmentImage encodes a garment sewing pattern's geometry, topology and placement into multi-channel regular grids. Machine learning models trained on GarmentImage achieve seamless transitions between patterns with different topologies and show better generalization capabilities compared to models trained on vector-based representation. We demonstrate the effectiveness of GarmentImage across three applications: pattern exploration in latent space, text-based pattern editing, and image-to-pattern prediction. The results show that GarmentImage achieves superior performance on these applications using only simple convolutional networks.

==> application.tex <==
\section{Application}

\subsection{Sketch-based Garment Modeling}
We built a sketch-based garment modeling application as an example of generative neural network using dress codes. The user paints a 2D garment on a T-pose human body as input, and the system generates a 3D surface model of the garment on the human model together with its 2D pattern as output. Figure shows some examples. It shows that the single model generates garments of diverse topology with fine details. 

We prepared a data set consisting of 150 dress codes consisting of shirts, skirts, and dresses with and without sleeves. 
We then reconstructed garment patterns, put them on a 3D human body, run cloth simulation, render them in gray-scale, and captured snapshots. We use a simple in-house cloth simulator based on position-based dynamics \cite{Muller2007} in this study. The pairs of a snapshot and a code are used as training data.

We used the basic dress code representation without extensions. The code side is 14x16x16, 7 values for each entry of each side. We dropped edge vectors of right and bottom edges to keep it compact (sacrificing precision). We convert a seam type into a four dimensional 1-hot vector before feeding a code into the network, so the tensor size of each code is 26x16x16. The network is a U-Net that takes a gray-scale image (1x16x16) as input and returns a dress code (26x16x16) as output (see Appendix C for details).

Figure shows the results. It successfully takes hand-painted rough sketches as input and returns 3D garments and 2D patterns with diverse topology, which is difficult for models trained for a specific topology \cite{Wang2018}. Figure shows that the model can generate patterns not contained in the training data (all patterns in the training data were symmetric), demonstrating its generalization capability. Figure shows that the system naturally blends patterns with different topology  (skirt with sing and multiple panels), which is difficult in classification based methods \cite{Korosteleva2022}. Figure shows a failure case. It generates a random result when the user draws something not included in the training data.


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figs/results.pdf}
  \caption{The results of sketch-to-pattern. Left: Input sketch, Middle: 3D garment after simulation, Right: Garment Pattern. The 2D layout of patterns is manual.}
\end{figure}

==> method_old.tex <==
%  This file is a version before takeo reorganize Method section

% \section{Method}
\section{\methodName}
\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{figs/GarmentImageConversion_v12.pdf}
  \caption{
  \ichao{We also need to update this caption after the content in main text is finalized.}
  \textbf{Encoding and decoding process.}
  A \methodName~is converted automatically from a sewing pattern in vector format (a).
  First, we stitch panels and fill the gap between them to rasterize the sewing pattern into (b) a bitmap representation.
  Through the rasterization process, we obtain grid edges in the bitmap that correspond to each edge on the original sewing pattern, which enables us to assign a seam type to each grid edge.
  Additionally, we gain the pairs of vertices on the boundary of the bitmap representation and the original sewing pattern.
  We finally compute the deformation matrices to match them.
  This is how we obtain inside/outside labels, seam types, and deformation information to construct \methodName.
  For the decoding process, we construct quad mesh from the grid cells in \methodName~and apply the deformations to reconstruct the sewing pattern.
 % \ann{(e) is confusing }\ichao{Yeah I think we can remove it?} 
 } 
  \label{fig:garmentImageConversion}
\end{figure*}

% \subsection{Representation}
\methodName~representation encodes a sewing pattern-including a discrete collection of 2D panels, stitching information, and the placement of each piece on the body—as raster data. 

%Each sewing pattern is represented by two separate grids: one for the front side and another for the back side. Each panel occupies several grid cells.

%The position of this set of cells on the 2D grid represents the position of the panel on the human body.


%and adjacency of seam edges represents the connectivity among the boundary curves



% where each cell contains three attributes: an inside/outside label, a local deformation, and seam types on its edges to define the panel shape and stitching information with other panels.





%\methodName~encodes a sewing pattern (panels, stitching information and placement of each piece on a body) as raster data, where each pattern is represented by two separate grids: one for the front side and another represent the back side of the sewing pattern.
% Specifically, \methodName represent a sewing pattern with multiple 2D panels as a bitmap representation composed of inside/outside flags, stitching, and deformation information.
%The sewing pattern is divided into 2D panels composed of grid cells.
%Each cell grid contains an inside/outside label, a local deformation, and seam types on the edges.%, which provides stitching information.
%\ann{I do not understand this sentence: Meanwhile, the edges of these grid cells provide stitching information, indicating how edges should be joined.}

As illustrated in~\cref{fig:garmentImageConversion}, \methodName can be automatically encoded from an existing vector-based sewing pattern \ann{is this vector-based sewing pattern clear at this point?}, and seamlessly decoded back into a vector-based format for downstream tasks. Besides, \methodName is able to represent a large variety of sewing patterns and design features such as waistbands, darts and panels with holes as illustrated in \cref{fig:complicated_garment}.
%Additionally, \methodName~can represent panels with holes, which is unachievable in the previous vector representation.
We describe the details of the \textit{encoding} and the \textit{decoding} process in the
following subsections.

%can be used to reconstruct the sewing pattern with stitching information.
% By decoding this representation, it is possible to reconstruct both the garment’s shape and its stitching.
%Next, we will describe the details of \methodName~representation, the \textit{encoding}, and the \textit{decoding} process.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/garmentimageconcept_v7.pdf}
%   \caption{
%   % \todo{Change ``NO STITCH'' to ``NON-STITCH''.}
%   \textbf{Overall concept of \methodName~representation.}
%   % A visualization of \methodName. 
%   Gray cells indicate that they are part of the garment. Dotted line patterns indicate seam types. A deformed quad inside each grid cell visualizes the deformation embedded in the cell.
%   \ann{need discussion. The geometric information in the garmentimage is not illustrated, what about e) in figure?}
%   }
%   \ichao{Yeah I think Yuki and I talked about this in slack, and I think something similar to (e) in~\cref{fig:encode_deform} is nice.
%   But the current ones in (e) in~\cref{fig:encode_deform} seem grid-dependent, we probably want one that can representation geometric info but easier to make.}
%   \label{fig:concept}
% \end{figure}

\subsection{Encoding}
Encoding process aims to derive the \methodName representation from the vector-based sewing pattern. In \methodName, each sewing
pattern is represented by two separate grids: one for the front side
and another for the back side. Each panel occupies several grid cells.
The position of this set of cells on the 2D grid represents the
position of the panel on the human body. 

To capture the panels’ shape and stitching information, we define three attributes for each grid cell: an inside/outside label, a local deformation matrix, and seam types. The stitching information is encoded as the adjacency relationships between seam types, while the panel's shape is embedded within the inside/outside label and deformation matrix. We provide a detailed explanation of these attributes as follows.




%To achieve this, we define three attributes for each grid cell


\subsubsection{Inside/Outside Label} This binary label indicates whether the grid cell is inside one of the 2D panels of a sewing pattern. 
%Each grid cell contains a binary value indicating whether it lies inside one of the 2D panels of a sewing pattern.
We begin by fixing one panel at \ann{where?} on the canvas, then align its connected panels with the corresponding stitched edges, making small adjustments to ensure proper edge alignment \ann{how, worth to mention?}. By recursively repeating this process, we determine the positions of all the panels. Finally, we rasterize the canvas into bitmap grid and
label the grid cell as inside if its centroid lies in the
one of the garment panels. In the rasterization process,  \setlength{\intextsep}{-1pt}  % Space above and below the figure
\setlength{\columnsep}{2pt} % Space to the right or left of the figure
\begin{wrapfigure}{r}{0.2\textwidth} 
    \centering
    \includegraphics[width=0.19\textwidth]{figs/mapping.png} % Replace 'example-image' with your image file name
    \label{fig:sliding}
\end{wrapfigure}
we also establish mapping $\Phi$ between each edge curve in the panel and its corresponding edges in the bitmap \ann{this mapping needs to be mentioned a few times, add a small inset like this but it is a detail, not sure?}. This mapping allows us to transfer the stitching information from the original sewing pattern to the edges in the bitmap as we detail below.



% In~\cref{fig:concept}(b), we only show cells with their inside label equals to TRUE.
\subsubsection{Seam Type}
The seam type of each edge in the grid cell is used to store stitching information.
We define four seam types \ann{i wonder shall we put small inset figures for this}:



%Each grid cell contains seam-type information for its left and bottom edges. 
%Overall, there are four seam types:
\begin{itemize}
\item \textbf{\nonBoundary}:  an internal edge inside a panel.
% with no stitching.
\item \textbf{\nonStitch}: a boundary edge with no stitching. %Note that a non-stitch edge may also appear within a panel. 
\item \textbf{\frontToBack}: an edge that is stitched to a corresponding edge on the opposite side (front-to-back). 
%The matching front-to-back edges must align in the same position on both sides. At least one of the two grid cells sharing this edge must be labeled as inside.
\item \textbf{\sideBySide}: an edge that is stitched to a corresponding edge on the same side (front-to-front, back-to-back). 
%Both grid cells sharing a side-by-side edge must be labeled as inside, which means they are inside different panels.
\end{itemize}

Using the mapping between each edge curve in the original panel and its corresponding edges in the bitmap we build in the rasterization process,  we can now assign a unique seam type from the four possible types to each edge within the grid cell.



\subsubsection{Deformation matrix}

The next step is to embed the geometry of the panel (shapes of
panel) into the grid. For each grid cell, we define a deformation matrix \( F \in \mathbb{R}^{2 \times 4} \) where each column represents a \textit{deformation vector} \( f \in \mathbb{R}^{2 \times 1} \), encoding the deformed relative position of the corresponding edge. We compute deformation vector by first construct a quad mesh $M=(V, E)$ by connecting grid cells associated with a panel, where $V$ is mesh vertices and $E$ is the mesh edges. We then deform the quad mesh so that its boundary matches with the boundary curves while minimizing the
edge deformation. We formulate this as a least square problem \cref{eq:encoding}: 
\begin{align}
     \argmin_{\bm{\bar{v}}} {\sum_{i,j \in E}((\bar{v}_j-\bar{v}_i) - (v_j-v_i))^2} + {\sum_{\bar{v_i} \in B} (\bar{v}_i-b_i)^2} ,
    \label{eq:encoding}
    \end{align}
where  $v_i$ and $\bar{v}_i$ are the positions of the $i$-th vertex of $M$ before and after deformation, $(i, j) \in E$ indicates that $v_i$ and $v_j$ are connected by an edge in $M$. $B$ is the set of boundary vertices forming $M$, and $b_i$ is the associated position on the panel curve of the boundary vertex. 

The deformation vector for edge, \( f_{ij} \), is computed as \( f_{ij} = \bar{v}_j - \bar{v}_i \). During decoding, the vector \( f_{i,j} \) is used to determine the optimal positions of the grid's vertices.
    
    %position of the sample point the boundary curve associated with the $i$-th vertex.

 %that specifies how its four edges should be deformed so that boundary edges of the panel can match with the original panel curves.

%Within this matrix, each column is a $(2,1)$ vector representing the deformed relative position of the corresponding edge.
%During encoding, the optimal matrix is computed and stored for each grid cell.
   
 %   The first term aims to preserve the local shape of each quad mesh by minimizing the difference between the edge vectors before and after deformation.
%    The second term minimizes the distance between mesh vertices and corresponding sample points on the boundary curves on the original sewing pattern. 
   % This formulation can be written in a matrix form $|Lv-B|^2$ for each dimension, and we obtain the optimal solution $\bm{v}^{*}$ as a solution of $(L^TL)\bm{v}^{*} = L^TB$. 

    

%deforming the grid so that its boundary conforms to the curve boundary of the input panel while minimizing the distortion of the quadrilateral elements (\cref{fig:encode_deform}).

%


\subsection{Decoding}
\label{sec:decoding}
The encoding process embeds a sewing pattern information onto \methodName, while the decoding process aims to recover the sewing pattern (panels, stitching information and placement of each piece on a body) from \methodName. With the embedded information on the grids, the decoding process is straightforward.
%a sewing pattern back to its vector-based representation (panels, stitching information and placement of each piece on a body) from \methodName~ 
%is straightforward with our formulation(\cref{fig:decoding}).
% This process takes a \methodName~as input and reconstructs 2D garment panels with stitching information (see \cref{fig:decoding}). 
We compute it in three steps:

\noindent\textbf{Panel Clustering}: First, different panels need to be separated from \methodName.
We group grid cells flagged as inside and enclosed by seam edges (i.e., grid cell edges with seam type \nonStitch, \frontToBack, \sideBySide). Each resulting group of grid cells corresponds to a distinct garment panel.


% , mirroring the encoding process.
\noindent\textbf{Panel shape recovery}: Next, for each identified panel, we aim to recover its shape. % from deformation matrix $F$.
We construct a quad mesh $M=(V, E)$ from the group of grid cells as that of in encoding, and deform the quad mesh $M$ to $\hat{M} = (\hat{V}, \hat{E})$. The deformation aims to minimize the difference between resulting edge $\hat{e}_{i,j} = \hat{v}_j-\hat{v}_i$,
 and embedded deformation vector $f_{i,j}$ while keeping the location of the resulting mesh on the grid. We formulate it as another least square problem:%so that each resulting edge in $\hat{M}$, $\hat{e}_{i,j} = \hat{v}_j-\hat{v}_i$, is as close as to the embedded deformation vector $f$. 
\begin{align}
 \argmin_{\bm{\hat{v}}} {\sum_{i,j \in E}((\hat{v}_j-\hat{v}_i) - f_{ij})^2} +  \sum_{v_i \in V}(\hat{v}_i - v_i )^2
\end{align}
where $v_i$ is the vertex position in $M$ (i.e., on the grid), $(i, j) \in E$ indicates that $v_i$ and $v_j$ are connected by an edge in $M$ and $f_{ij}$ is its encoded deformation vector. 


\noindent \textbf{Stitching and placement recovery} With the recovered panel shape, to get the stitching information, we can transfer edge types from the grid to the correspondence deformed edges on the panel curves through the mapping $\Phi$.  The position of the panel's quad mesh in the grid represents the position of the panel on the human body. One can easily construct a 3D garment mesh around a 3D human body and run a physical simulation, or print and stitch 2D patterns to create a physical garment.

%For the grid cells of each identified panel, we construct a quad mesh by connecting the relevant grid cells according to the seam type on the edges. Each quad mesh is then deformed to reconstruct the shape of garment panel by solving the following optimization problem: 
% Differential geometry processing is employed to minimize distortion, ensuring that the resulting mesh represents the desired panel shape.
% This is achieved by solving the following minimization problem to compute the vertex coordinates \( \mathbf{v} \) of the mesh:

\subsection{Examples}
\methodName~can represent a garment sewing pattern by storing labels and deformation information in the cell grids. In \cref{fig:complicated_garment}, we show that this representation is able to represent a large variety of sewing patterns and design features such as waistbands and
darts. Additionally, \methodName can represent panels with holes, a capability that would require dedicated templates in a vector-based representation.
%In \cref{sec:encoding}, we demonstrate the case of a dress with sleeves, but \methodName~is able to handle other types of garments or features such as pants, waistbands, and darts as illustrated in \cref{fig:complicated_garment}.
%Additionally, \methodName~can represent panels with holes, which is unachievable in the previous vector representation.
\begin{figure}[t]
  \includegraphics[width=\linewidth]{figs/complicated_garment_v9.pdf}
  \caption{
  \textbf{\methodName examples.}
  % A visualization of \methodName. 
  \methodName can handle diverse garments and features such as darts (a) waistbands (c), and holes (d) and (e). 
  % \ann{put a,b,c plz, and for the holes case, can you put the vector representation (vectorized the third row)}
}
  \label{fig:complicated_garment}
\end{figure}


\begin{comment}
\subsection{Encoding}
\label{sec:encoding}
\ichao{What is the purpose of separating the descriptions of constructing \methodName~representation here and in~\cref{sec:dataset}?}
In the encoding process, an input sewing pattern is transformed into \methodName~representation.
This transformation consists of two parts: Deriving labels and computing deformation matrices.

\subsubsection{Deriving labels}
\label{sec:deriving_labels}
The transformation requires inside/outside labels and seam-type labels for each grid cell to construct meshes for each panel.
Additionally, boundary conditions that ensure each vertex on the \methodName~boundary aligns with the corresponding vertex on the target garment's boundary are necessary.
These labels and boundary conditions can be determined manually or automatically, with the automatic derivation method detailed in the experiment section.

We demonstrate this automatic process using a dress with sleeves, though the same approach applies to other garment types (see supplementary material for details).
We begin by aligning panels with their stitched edges by adjusting sleeve panel edges to match the corresponding edges on the main body panel.
Note that we align stitched edges for connecting the corresponding front and back panels so that \methodName~handles \frontToBack~seams properly.
Next, we rasterize the garment pattern into bitmap grids by labeling the grid as inside if the centroid of the grid is within the target garment panel. 

We then incorporate stitching details by assigning seam types to edges.
We know pairs between an edge in the original sewing pattern and its corresponding boundary edges in the bitmap through the rasterization process.
Therefore we can assign the seam type of the original sewing pattern to each edge in the bitmap.
If two stitched edges belong to opposite sides (front vs.\ back), we label them as \frontToBack.
When stitched edges are on the same side (front–front or back–back), we use \sideBySide~if they lie on different panels and \nonStitch~if they belong to the same panel.
All other boundary edges are labeled \nonStitch, and any remaining interior edges are labeled \inside.
This process yields inside/outside labels and seam types for each grid cell.

Next, we register vertices on the \methodName~boundary to corresponding points on the original garment boundary (before realigning stitched edges).
Specifically, we know the boundary vertex of the \methodName~representation corresponding to an original sewing pattern vertex.
We then assign the remaining boundary vertices of the \methodName~to sampled points along the original sewing pattern edges.
In this way, we derive the inside/outside flags, seam types, and boundary conditions.

\subsubsection{Computing Deformations}
\label{sec:computing_deformations}
Given the labels and boundary conditions gained in \cref{sec:deriving_labels}, the encoding process next involves deforming the grid so that its boundary conforms to the curve boundary of the input panel while minimizing the distortion of the quadrilateral elements (\cref{fig:encode_deform}).
The steps are as follows:
\def\theenumi{\Roman{enumi}}
\def\labelenumi{\theenumi)}
\begin{enumerate}
    \item \textbf{Quad Mesh Construction}: The system begins by constructing a quad mesh $M=(V, E, F)$ by connecting grid cells that belong to the same panel by referring to the inside/outside labels and seam type labels.
    \item \textbf{Mesh Deformation}: The quad mesh is then deformed to match the boundary curves of panels in the input sewing pattern by solving the following optimization problem:
    % garment panel. 
    % This deformation minimizes edge distortion by solving the following optimization problem:
    \begin{align}
    \bm{v}^{*} = \argmin_{\bm{v}} ( \tcboxmath[colback=white,colframe=purpleD,title=shape preservation]{\sum_{i,j \in E}((\bar{v}_j-\bar{v}_i) - (v_j-v_i)^2)} + \tcboxmath[colback=white,colframe=greenD,title=boundary]{\sum_{i \in B} (\bar{v}_i-b_i)^2} ),
    \label{eq:encoding}
    \end{align}
    where $B$ is the set of sample points on the boundary curves, $v_i$ and $\bar{v}_i$ are the positions of the $i$-th vertex of $M$ before and after deformation, and $b_i$ is the position of the sample point the boundary curve associated with the $i$-th vertex.
    The first term aims to preserve the local shape of each quad mesh by minimizing the difference between the edge vectors before and after deformation.
    The second term minimizes the distance between mesh vertices and corresponding sample points on the boundary curves on the original sewing pattern. 
    This formulation can be written in a matrix form $|Lv-B|^2$ for each dimension, and we obtain the optimal solution $\bm{v}^{*}$ as a solution of $(L^TL)\bm{v}^{*} = L^TB$. 
\end{enumerate}





% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/screenshot.pdf}
%   \caption{\ichao{Maybe replace this?}A screenshot of the encoding tool. The user manually embeds front and back pieces into grids.}
% \end{figure}

 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/encoding.pdf}
%   \caption{Computation and embedding of local deformation.  The system deforms the quad mesh so that its boundary matches with the boundary curves of the pattern piece. The amount of deformation of each quad face is stored in the corresponding  grid cell.}
%   \label{fig:encode_deform}
% \end{figure}


\subsection{Decoding}
\label{sec:decoding}
Reconstructing a sewing pattern by decoding a \methodName~can also be performed automatically (\cref{fig:decoding}).
% This process takes a \methodName~as input and reconstructs 2D garment panels with stitching information (see \cref{fig:decoding}). 
The decoding procedure includes the following steps:
\begin{enumerate}
\item \textbf{Panel Clustering}: \ichao{It is a bit confusing what does it mean by ``surrounded by seam edges''.} Our method identifies and clusters grid cells flagged as inside and surrounded by seam edges (i.e., grid edges labeled with seam types other than \nonStitch). 
Each cluster represents a distinct garment panel.
\item \textbf{Quad Mesh Construction}:
For each identified panel, the system constructs a quad mesh by connecting the relevant grid cells according to the seam type on the edges.
% , mirroring the encoding process.
\item \textbf{Deformation}:
Each quad mesh is then deformed to reconstruct the shape of garment panel by solving the following optimization problem: 
% Differential geometry processing is employed to minimize distortion, ensuring that the resulting mesh represents the desired panel shape.
% This is achieved by solving the following minimization problem to compute the vertex coordinates \( \mathbf{v} \) of the mesh:
\begin{align}
\bm{v}^{*} = \argmin_{\bm{v}} (\tcboxmath[colback=white,colframe=purpleD,title=shape recovery]{\sum_{i,j \in E}((\bar{v}_j-\bar{v}_i) - vec_{ij})^2)} +  \tcboxmath[colback=white,colframe=greenD,title=fix location]{\sum_{i \in V}(\bar{v}_i - g_i )^2} )
\end{align}
where $E$ is the mesh edges, $V$ is mesh vertices, $vec_{ij}$ is encoded edge vector, $g_i$ is the position of $v_i$ on the grid before deformation. 
The first term minimizes the difference between the resulting edge vector and embedded edge vectors. 
\ichao{I think we only need to compute the second term using a subset of vertices right? 
I.e., it should not use $i\in V$?}
\yuki{Yeah, I think so. Let me think about this more.}
The second term keeps the location of the resulting mesh on the grid. 
Again, this can be written in a matrix form $|Lx-B|^2$ for each dimension, and we obtain $x$ as a solution of $(L^TL)x = L^TB$.

\end{enumerate}


 
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/decoding.pdf}
%   \caption{Reconstruction of 2D garment pieces from a dress code. 1) clustering of inside faces. 2) construction of a quad mesh. 3) Deformation of the quad mesh.} 
%   \label{fig:decoding}
% \end{figure}

 \end{comment}
